WikiPassageQA: A Benchmark Collection for Research on Non-factoid Answer Passage Retrieval

With the rise in mobile and voice search, answer passage retrieval acts as a critical component of an effective information retrieval system for open domain question answering. Currently, there are no comparable collections that address non-factoid question answering within larger documents while simultaneously providing enough examples sufficient to train a deep neural network. In this paper, we introduce a new Wikipedia based collection specific for non-factoid answer passage retrieval containing thousands of questions with annotated answers and show benchmark results on a variety of state of the art neural architectures and retrieval models. The experimental results demonstrate the unique challenges presented by answer passage retrieval within topically relevant documents for future research.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-siggraph.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-siggraph.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> introduction.tex <==
The advent of deep learning has allowed recent work in numerous fields to achieve state of the art performance on key tasks, with larger networks often outperforming equivalent smaller networks after accounting for overfitting.
However, these deep neural networks contain millions parameters after only a small number of layers which necessitates a large amount of training data when compared to more conventional models.
As such, high quality openly available benchmark data sets are critical for research progress. \dan{cite this} ImageNet, TREC, GOV2, MNIST, and others allow the community to not only rapidly develop new models for a task, but to incrementally learn how a model interacts for a specific task.

With the rise in mobile and voice assisted search, there is a growing need to develop models capable of responding to the task of answer passage retrieval, where 




\iffalse
!!This is a rough draft/prose road map, I'll have it flow better on a rewrite!!

- Rise in mobile search and voice assistance
- Deep learning has allowed the for effective Answer retrieval system
    - WikiQA, InsuranceQA, MARCO don't address the passage retrieval problem
        - wikiQA: sentences, factoid in nature
        - InsuranceQA

Outline and key points 

1. High quality open available benchmark data sets are critical for research progress on various IR tasks. For instance, ImageNet, TREC GOV2, CLUE Web, SQUAD, etc...

2. In terms of question answering, there are some existing benchmark data sets including TREC QA, Wiki QA, Insurance QA... But most of these data sets are on factoid question answering and the answers are short snippets or sentences on answer facts. There is a lack of high quality non-factoid question answering data sets.

3. To address this issue, WebAP was released as an initial effort for ... But the number of questions of WebAP is not enough to train powerful deep learning models. There are no previous large non-factoid QA data sets with thousands of questions...

4. Thus in this paper, we propose ...
